WebWISE: Web Interface Control and Sequential Exploration with Large Language Models

The paper investigates using a Large Language Model (LLM) to automatically perform web software tasks using click, scroll, and text input operations. Previous approaches, such as reinforcement learning (RL) or imitation learning, are inefficient to train and task-specific. Our method uses filtered Document Object Model (DOM) elements as observations and performs tasks step-by-step, sequentially generating small programs based on the current observations. We use in-context learning, either benefiting from a single manually provided example, or an automatically generated example based on a successful zero-shot trial. We evaluate the proposed method on the MiniWob++ benchmark. With only one in-context example, our WebWISE method achieves similar or better performance than other methods that require many demonstrations or trials.

==> commented_out_text.tex <==
%  to generate programs leverages the in-context learning ability of  Large Language Models (LLM) to generate programs by taking the Document Object Model (DOM) element as the observation of the web-based computer tasks.
% Automating control of software interfaces and web pages offers significant advantages, including enhanced efficiency, error reduction, and improved accessibility. Traditional approaches, such as Reinforcement Learning (RL) and Imitation Learning, face limitations due to extensive data requirements and the excessing training time. In contrast, Large Language Models (LLMs) like GPT demonstrate exceptional learning capabilities but encounter challenges in controlling software and web interfaces due to shortcomings in environment grounding and sequential decision-making. In this paper, we propose a methodology that leverages LLMs' prior knowledge to generate context-aware, adaptive programs via exploration(sequentially refined) for AI tasks related to automated software and web page control. Our approach addresses environment grounding by extracting and processing pertinent information from the environment (DOM Elements) and integrating it with LLMs. Additionally, we introduce an iterative technique for sequential decision-making. Furthermore, we investigate an initial warm-up phase that allows LLMs to explore the solution space without in-context examples, generating correct programs to guide subsequent iterations. Our research contributes to the AI field by enhancing LLMs' performance in software control tasks, expanding their applicability, and revealing new opportunities for future exploration.


%Software control requires a sequence of actions and observations rather than a single-shot solution. LLMs conventionally generate an entire program in a single step, without considering the impact of their actions on the environment. To address this issue, we introduce an approach that allows LLMs to iteratively generate individual, feasible actions and refine their decision-making based on observed changes in the environment. This method enhances LLMs' ability to understand the consequences of their actions, adapt their subsequent decisions, and ultimately improve their performance in embodied tasks.

% \section{Introduction(3)}
% The control of software interfaces that emulate embodied environments necessitates agents capable of perceiving, understanding, and interacting with their surroundings. Automating the control of software and web pages offers numerous benefits, such as increased efficiency, reduced human error, and the ability to perform tasks beyond human capabilities. Furthermore, automated control can improve accessibility for individuals with disabilities and facilitate the development of intelligent systems that can adapt to a wide range of applications.

% In this context, Reinforcement Learning (RL) and Imitation Learning have traditionally been employed to address such tasks. However, RL methods often face limitations due to their extensive data requirements, numerous iterations needed for convergence, and the complexity of crafting task-specific reward functions, ultimately restricting their scalability and generalizability. A significant factor contributing to these limitations is their lack of a priori world knowledge.


% In contrast, Large Language Models (LLMs) such as GPT display a unique advantage in their ability to incorporate world knowledge or human priors acquired during the training process. This integration allows LLMs to demonstrate remarkable zero-shot or few-shot learning capabilities across various problem domains, excelling in tasks related to natural language understanding, planning, reasoning, and more. Despite these successes, LLMs continue to face substantial challenges when attempting to control software or web interfaces due to several shortcomings:

% \textbf{Environment Grounding}: To generate programs that take into account both the query and the environment's content, such as images or other sensory data, LLMs must overcome their tendency to produce programs solely based on the query. We propose a novel method that extracts and processes pertinent information from the environment (DOM Elements) and incorporates it into LLMs, enabling the creation of context-aware and environment-sensitive programs that improve LLMs' performance in embodied tasks.

% \textbf{Sequential Decision-Making}: Software control requires a sequence of actions and observations rather than a single-shot solution. LLMs conventionally generate an entire program in a single step, without considering the impact of their actions on the environment. To address this issue, we introduce an approach that allows LLMs to iteratively generate individual, feasible actions and refine their decision-making based on observed changes in the environment. This method enhances LLMs' ability to understand the consequences of their actions, adapt their subsequent decisions, and ultimately improve their performance in embodied tasks.

% Additionally, we suggest an initial warm-up phase, during which LLMs undergo ten iterations, allowing them to explore the solution space and generate one or two correct programs to inform subsequent iterations. This exploratory strategy equips LLMs to search for appropriate prompts and generate more interpretable and generalizable policies for embodied tasks, potentially circumventing the need for labor-intensive manual provision of few-shot examples.

% In this paper, we present a novel approach that capitalizes on the strengths of LLMs to generate context-aware, sequentially-refined programs for embodied AI tasks. By addressing the challenges of environment grounding and sequential decision-making, our method enhances LLMs' performance in embodied tasks. Our work contributes to the ongoing progress in AI research, broadening the range of LLMs' applications and unveiling new avenues for future investigation.

% \section{Introduction (2)}
% Large Language Models (LLM) have successfully been used in many different applications and domains. One such application is generating code to perform various tasks, like in VisProg and ProgPrompt. In both VisProg and ProgPrompt, prompts are formed by combining new instructions with several in-context examples containing Python code for similar tasks. While such an approach works for typical vision-language tasks, it fails for more complex tasks, such as automating computer tasks. 

% Performing automated computer tasks requires executing actions that are admissible for both the general system (the computer) and the content on the screen. Two shortcomings of Vis-Prog type methods that make automated computer tasks difficult  is the lack of visual information and single-shot generation. Since VQA questions are generally of the same form, previous question examples are enough to generate code. However, for tasks where instruction prompts do not contain all necessary information, such approaches fail like in automated computer tasks. Vis-Prog-type (need a name for this) methods generate code for a task all at once which makes performing sequential decision-making difficult. For example, (insert automating computer task where there is a change that changes code)

% In our paper, we present a method for automating web computer tasks with LLMs. Our method uses a visual summary of HTML pages and performs actions step-by-step (we should figure out a way to say this so it is not confused with the original step by step paper).  



% \section{Introduction}
% Embodied AI, which involves agents that can perceive, understand, and interact with their environment, has gained significant traction in the field of artificial intelligence research. Large Language Models (LLMs) such as GPT have demonstrated remarkable success in various tasks, encompassing natural language understanding, planning, reasoning, and more. Despite these achievements, LLMs still face considerable challenges when tackling embodied AI tasks, which are primarily addressed through reinforcement learning (RL) techniques, including behavioral cloning, imitation learning, and others. While RL methods have shown promise, they are often hindered by the need for extensive data, numerous iterations for convergence, and the complexity of designing task-specific reward functions, limiting their scalability and generalizability.

% A distinctive advantage of LLMs is their capacity to integrate world knowledge or human priors, which they acquire during the training process. This incorporation enables LLMs to exhibit impressive zero-shot or few-shot learning capabilities in various problem domains. However, LLMs underperform in embodied tasks due to two primary shortcomings:

% Environment grounding: LLMs must be capable of generating programs that consider both the query and the environment's content, such as images or other sensory data. Existing LLMs generate programs based on the query alone, disregarding the environment's content. To tackle this challenge, we introduce a method that extracts and processes relevant information from the environment and feeds it to the LLMs. This approach enables the generation of more context-aware and environment-sensitive programs, enhancing the LLMs' performance in embodied tasks.

% Sequential decision-making: Many embodied tasks necessitate a series of actions and observations, as opposed to a single-shot solution. LLMs typically generate an entire program in one step, without considering the consequences of their actions on the environment. To surmount this limitation, we develop an approach that allows LLMs to generate individual, feasible actions iteratively, refining their decision-making based on the observed changes in the environment. This method enables LLMs to better comprehend the impact of their actions, adjust their subsequent decisions, and ultimately improve their performance in embodied tasks.

% Furthermore, we propose an initial warm-up phase, during which the LLMs are run for ten iterations. This phase allows the models to explore the solution space and generate one or two correct programs, which can subsequently guide the following iterations. This exploratory strategy empowers LLMs to search for suitable prompts and generate more interpretable and generalizable policies for embodied tasks.

% In this paper, we present an innovative approach that leverages the strengths of LLMs to generate context-aware, sequentially-refined programs for embodied AI tasks. By addressing the challenges of environment grounding and sequential decision-making, our method enables LLMs to achieve enhanced performance in embodied tasks. Our work contributes to the ongoing advancements in AI research, expanding the scope of LLMs' applicability and uncovering new possibilities for future studies.


% As highlighted in \cite{}, LLMs similarly harness extensive world knowledge, which enables them to effectively solve tasks with only a few examples, echoing the efficiency of human performance in complex video games. Thus, LLMs exhibit impressive zero-shot capabilities 
%  A popular benchmark for evaluating these methods in web interface is the MiniWob++ (insert mini wob ++ citation) which is an extension of the Mini Wob benchmark(citation). While RL-only approaches are able to achieve human-level performance, fgeg involve large amount of annotated training data and extensive training data
% Reinforcement Learning (RL) is another successful method in computer task automation. \cite{silver16}\cite{Mnih2015HumanlevelCT} 
% Reinforcement Learning (RL) has been another popular paradigm demonstrating remarkable success in learning and mastering complex games.
%  In RL, an agent learns to perform actions in an environment to maximize the cumulative reward it receives. Recently, there has been growing interest in applying RL to web interface tasks. Web interfaces present unique challenges, such as varying layouts, dynamic content, and understanding user intentions. \cite{} proposed <>, an RL-based framework for web automation tasks, such as form filling and web navigation. Their approach allowed agents to learn and generalize across different websites, demonstrating the potential of RL in web interface tasks. 


% CCNet: A Data-Driven Approach for Learning to Control Computers- uses behavior cloning plus designs architexture \\

% RL Wob Papers:
% - Improving Policy Learning via Language Dynamics Distillation: pre-trains with language, finetunes on RL \\
% - WebShop: Towards Scalable Real-World Web Interaction with Grounded Language Agents: develops imitation learning+RL for web shop task \\

% - Automatic Web Testing Using Curiosity-Driven Reinforcement Learning: policy learning \\
% - Mapping Natural Language Instructions to Mobile UI Action Sequences: decouples language and actions \\
% - Learning to navigate the web: decompose steps, curriculum learning \\
% - Reinforcement Learning on Web Interfaces Using Workflow-Guided Exploration: constrains exploration (workflow); RL approach 
% - 

% RL+LLM: Grounding large language models in interactive environments with online reinforcement learning \\
% LLM Action papers:
% - Language models as zero-shot planners: Extracting actionable knowledge for embodied agents: decompose high level plans and get admissible actions \\
% Followup: Inner monologue: Embodied reasoning through planning with language models: reason over feedback \\
% - (Robots) Do as I can, not as I say: Grounding language in robotic affordances: language models provide high level knowledge combined with low level skills from a robot \\
% -  Socratic models: Composing zero-shot multimodal reasoning with language: shows how different pre-trained models communicate \\

% Generating Code (for visual tasks) from LLMs
% - Visual Programming: Compositional visual reasoning without training \\
% - Progprompt: Generating situated robot task plans using large language models. \\
% - Visual ChatGPT: Talking, Drawing and Editing with Visual Foundation Models \\
% - ViperGPT: Visual Inference via Python Execution for Reasoning \\
% - Language Models are Few-Shot Learners \\

% Can include like one sentence about 'reasoning with prompting': 
% - General work on reasoning: 
%     - Chain-of-Thought Prompting Elicits Reasoning in Large Language Models \\
%     - Large language models are zero-shot reasoners. \\
%     - Show your work: Scratchpads for intermediate computation with language models. 
% - Reasnonig and action together: 
%     - ReAct: Synergizing Reasoning and Acting in Language Models
%     - Using a simulationn: Mind's Eye: Grounded Language Model Reasoning through Simulation
% - Other reasoning:
    % - Self-Consistency Improves Chain of Thought Reasoning in Language Models: new decoding strategy 
    % - Text and Patterns: For Effective Chain of Thought, It Takes Two to Tango: strategies  for prompting 
    % - STaR: Bootstrapping Reasoning With Reasoning: bootstrap examples with more examples 
    % - Chain of Thought Imitation with Procedure Cloning: imitation learning plus chain of thought 
    % - Recitation Augmented Language Models: samples from memory to add to curren tcontext 
   % - Reflexion: an autonomous agent with dynamic memory and self-reflection


   
% For our methods, we uses the Python interface to interact with different tasks, which follows the Gymnasium API and Selenium Webdriver to execute different actions on the web interfaces. For each task, the interface will contain the natural language description of the task and information of the visual objects shown on the task interface.

% We first describe the problem formulation, how WebWISE interprets observations from the web environment, 


% we discuss how LLMs can function as interactive problem solvers by integrating observations from web interface environments into context-aware planning using our proposed methodology, WebWISE.



% The observation $o$ may be success detection, failure detection, DOM Elements (which can be a proxy for object detection, scene description, etc.). Our work studies to what extent the LLM planner is able to reason over and utilize such feedback to "close the loop" with the environment and improve planning and solving the task in zero-shot.

% The goal of our work is to investigate the capability of the LLM planner to effectively reason over and utilize the feedback $f$ and observation $o$ to enhance planning and task-solving performance in a zero-shot setting. 

% We formulate WebWISE by injecting feedback from the environment in the form of DOM elements into the LLMs language prompts as the agent interacts with the environment. While LLMs have demonstrated exceptional planning abilities on a 

 


% Remember to mention the regex, prompts

% - Baseline 1: given task description, no DOM elements, prompt w/functions \\
% - Baseline 2: DOM elements, task description, prompt with functions\\
%             - No example\\
%             - With example\\
% - Baseline 3: DOM elements, task description, feedback of DOM elements, prompts with functions\\
% - Baseline 4: Warmup cycle gives sample solution figuring out  by itself (Including DOM elements, task description, and solutions), DOM elements, task description, prompt with functions\\

% To ensure fair evaluation across all tasks, we used the same Language Model (LLM) for all baselines. Specifically, we employed ChatGPT \cite{} or 'gpt-3.5-turbo' provided by OpenAI through API. To prevent any bias, we created a list containing the initial prompts, predefined functions, task description, and observations of the task interface for each iteration of each task. This ensured that no previous solution was utilized as a reference. For our model, we set the temperature to 0 and the maximum number of tokens that can be fed into our model to 4096.



% If the complete indicator is  (i.e. the task was solved correctly) then the cycle ends. Otherwise the cycle continues until $s$ is true or time runs out. For example, the next cycle would use the new observable DOM elements $d_{t+2}$ to generate a program $x_{t+2}$ = $\pi(nl,d_{t+1})$, using the same instruction $nl$ and the updated DOM elements $d_{t+2}$. The execution engine then applies the program through $\phi(x_{t+2})$, resulting in a new success indicator $s$ and observations $d_{t+2}$.  This framework is versatile and can be generalized to various tasks, including single-step, multi-step, logical reasoning, and exploratory tasks.

% In contrast, prior works \cite{Gupta2022VisProg}\cite{surís2023vipergpt} generate the program ${x}$ based exclusively on the query $i$, without conditioning it on the observations $d$. Additionally, they produce the entire program $x$ in one step, without considering environment changes at different time steps, $d_{tn}$.


% This agent is only capable of executing actions from a library of predefined API calls with short language descriptions $k$. The "planner," which is a pre-trained LLM[], attempts to find a sequence of skills/actions to accomplish the instruction. To observe the environment, the planner has access to textual feedback $f$ from the environment in the form of DOM elements that can be appended to the instruction. An action is then generated and executed based on the full instruction.


% \subsection{Interpreting Observations}
% The "state" of the interactive web environment can be given in both HTML form and/or with Domain Object Model (DOM) element form. For WebWISE, we use a modified version of the DOM elements. We create a summary of the DOM elements by extracting a pre-defined list of tags and classes. The DOM summary is added to the none-task specific prompt template. Similar to visual programming, our prompt consists of a small set of pre-defined Python functions that execute actions within the environment. A short description of each function is included as well as an example of how the function is used.

% \subsection{Environment Interaction}
% The actions to execute in the environment come from the output of the LLM. We use a regular expression to parse the output into acceptable Python code. After an action is performed, the DOM elements (and summary) are updated. For single-step tasks, if the correct action is performed, then the task is over. If the action is incorrect or it is a multi-step task, more actions are generated. 

% \subsection{Environment Feedback}
% Subsequent actions are generation the same ways as the initial action with the prompt appended with the DOM summary and task instruction. 


% \begin{algorithm}[H]
% \caption{Algorithm for WebWISE(l, k)}
% \begin{algorithmic}[1]
% \State \textbf{Input:} Task Description $l$, API $a$, in-context example $e$\\
% \State Get the initial observation space
% \State Extract DOM elements ${d}_{t+1}$ in initial observation state
% \State Generate program: ${x}_{t+1} = \pi(l,{d}_{t+1}, a, e)$ \Comment{Using program generator $\pi$ (e.g., LLM)} \\
% \State Apply execution engine: $r = \lambda({x}_{t+1})$ \Comment{Obtain reward $r$} \\
% \While{time not expired and reward != 0}
%         \State Obtain new observable DOM elements: ${d}_{t+2}$ \Comment{In next state of environment}
%         \State Generate program: ${x}{t+2} = \pi(i,{d}_{t+2})$ \Comment{Using program generator $\pi$ with same query and ${d}{t2}$}
%         \State Apply execution engine: $r = \lambda({x}_{t2},{d}_{t2})$ \Comment{Obtain reward $r$, observations ${d}_{t3}$}
%         \State $t1 \leftarrow t2$, ${d}_{t1} \leftarrow {d}_{t2}$
% \EndWhile
% \State \textbf{Output:} Task succeeds/fails
% \end{algorithmic}
% \end{algorithm}
    % \State Get the initial observation space
    % \State Extract DOM elements ${d}_{t+1}$ in initial observation state
    % \State Generate program: ${x}_{t+1} = \pi(l,{d}_{t+1}, a, e)$ \\
    % \While{$t+1$ > time limit and reward == 0}
    %     \State Apply execution engine: $r = \lambda({x}_{t+i})$ \Comment{Obtain reward $r$} \\
    %     \If{r != 0}
    %         \State break
    %     \State $i+=1$
    %     \State Get the current observation space after executing $x$
    %     \State Extract and update DOM elements ${d}_{t+i}$ in current observation state
    %     \State Generate program: ${x}_{t+i} = \pi(l,{d}_{t+i}, a, e)$
    % \EndWhile
    % \State \textbf{output} Reward $r$




%Comments (5/15):
% mention RCI 

%methods 
% problem formulation
% main method 
%'warmup' or self-training or context learning 
% problem should not include method instead of what task is, what we are provided, what we should produce
% describe warmup method 
% API  should be a seperate box (for diagram) (Check)
% say time out for figure (Check)
% d_0, d_1 in algorithm 
% example figure single step vs multi-step 
% example should show initial state, dom elements, execution, output generated program and result 
% k in-context examples (set of 0 to i-1) 
% make sucess s 
% use pi for program 
% list out API
% describe warmup method 

%discussion 
% scatter plot for one method vs another method 
% up to three scatter plots 


% \paragraph{Program Generation}
% We use a LLM as our program generator $\pi$. The input to the LLM is a prompt with 4 parts: DOM element summary, API $a$, task instruction, and in-context example(s) $e$. We use a function $getSummary$ that takes as the input all of the DOM element (for that task) and returns a subset of the element that belong to a pre-defined list of tags and classes. Our API $a$ is constant across all tasks and contains pre-defined functions that execute actions within Mini-Wob++. We use in-context examples as in GPT-3~\cite{brown2020language}. Each example contains an example input and output which is a string of Python code.


% \paragraph{Program Execution} 
% Once a program $x_t$ is generated, we need to execute it using the execution engine $\phi$.  H At this point, the 'Text+DOM' method finishes. An example of such an execution can be seen in Figure \ref{fig:text+dom}. 

% \paragraph{WebWISE}
% In WebWISE, programs are continuously generated and executed until either the task has been completed (the success indicator is ture) or the time to solve the task runs out. The WebWISE algorithm can be seen in Algorithm \ref{alg:webwise}. Programs are generated and executed in the same way as before. Note that the DOM summary used on the$i+1$st iteration has been updated based on the program generated and executed in the $i$th iteration. At any time step $n$, the $x_{t+n}$th program can either extend previous program lines or introduce semantically new ones. Programs are generated incrementally while accounting for both initial conditions and environment changes resulting from the agent's actions. For single-step Mini-Wob++ tasks, WebWISE allows for `self-correction' if the initial program generated is incorrect. Compared to Text+DOM, WebWISE enables Mini-Wob++ tasks that require multiple actions, to be performed in a step-by-step fashion. This difference is illustrated in Figures \ref{fig:text+dom} and \ref{fig:webwise}. In Figure \ref{fig:text+dom}, to complete a task correctly, an entire program has to be generated based on a single set of DOM elements.  In Figure \ref{fig:webwise}, the generated programs are smaller and are generated based on different sets of DOM elements. 


% \paragraph{Warmup Method}
% TODO  


% We can draw several observations based on the results:
% \begin{itemize}
%     \item \textbf{DOM Elements are not always needed} In the results table, the general difficulty of the task increases from left to right. We can see that for the easiest tasks, the Text Only method with a single in-context example is only 3\% lower than Text+DOM and WebWISE, which have the same performance. For single function tasks, the required action can be inferred from the task description and a single example. 
%     \item The hardest group of tasks, where the number of tasks requires, is also the group where updated DOM elements make the most difference. Tasks in this group generally require changing screens (e.g. the target button is not visible initially).The previous methods have no way of obtaining such information since the DOM elements are fixed.
%     \item The performance of Warmup WebWise is higher or around Text+DOM for $k=0$ but still behind $k=1$. For many of the tasks, no correct example was found during warmup period so the performance would be the same as the $k=0$ baseline. If a correct example was found, then the Warmup method was generally able to complete the task. 
% \end{itemize}


For simple tasks which requires just one function call , we outperform WebNT5-3B benchmark by a slight margin of $14.11\%$ which employs a finetuned large language model with 12K expert demonstration data.



specific and does not always work pertaining to this benchmark heuristically, however this proceed can be made adpative since the required sub set of DOM elements is task specific and it might be difficut to develop a fucntion that fits for all tasks

 most LLM based approaches, developing a robust prompting method would be a significant contribution.



     % & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 100\%                   \\ \hline
% click-button                & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 100\%                   \\ \hline
% click-checkboxes-large      & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{4\%}   & \multicolumn{1}{l|}{26\%}  & \multicolumn{1}{l|}{90\%}  & \multicolumn{1}{l|}{TLE}   & \multicolumn{1}{l|}{TLE}   & \multicolumn{1}{l|}{46\%,}    & \multicolumn{1}{l|}{100\%} & 89\%                    \\ \hline
% click-checkboxes-soft       & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{61\%}  & \multicolumn{1}{l|}{70\%}  & \multicolumn{1}{l|}{18\%}  & \multicolumn{1}{l|}{41\%}  & \multicolumn{1}{l|}{62\%}     & \multicolumn{1}{l|}{78\%}  & 86\%                    \\ \hline
% click-checkboxes-transfer   & \multicolumn{1}{l|}{4\%}   & \multicolumn{1}{l|}{28\%}  & \multicolumn{1}{l|}{66\%}  & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{52\%}  & \multicolumn{1}{l|}{TLE}   & \multicolumn{1}{l|}{73\%}     & \multicolumn{1}{l|}{100\%} & 99\%                    \\ \hline
% click-checkbox              & \multicolumn{1}{l|}{8\%}   & \multicolumn{1}{l|}{8\%}   & \multicolumn{1}{l|}{58\%}  & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{51\%}  & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{64.00\%}  & \multicolumn{1}{l|}{100\%} & 97\%                    \\ \hline
% click-collapsible-2         & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}      & \multicolumn{1}{l|}{66\%}  & 12\%                    \\ \hline
% click-collapsible           & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{2\%}   & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{96\%}  & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 100\%                   \\ \hline
% click-dialog-2              & \multicolumn{1}{l|}{64\%}  & \multicolumn{1}{l|}{70\%}  & \multicolumn{1}{l|}{70\%}  & \multicolumn{1}{l|}{72\%}  & \multicolumn{1}{l|}{68\%}  & \multicolumn{1}{l|}{54\%}  & \multicolumn{1}{l|}{78\%}     & \multicolumn{1}{l|}{74\%}  & 71\%                    \\ \hline
% click-dialog                & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{88\%}  & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 100\%                   \\ \hline
% click-link                  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{88\%}  & \multicolumn{1}{l|}{96\%}  & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{88\%}  & \multicolumn{1}{l|}{92\%}  & \multicolumn{1}{l|}{98\%}     & \multicolumn{1}{l|}{100\%} & 97\%                    \\ \hline
% click-option                & \multicolumn{1}{l|}{18\%}  & \multicolumn{1}{l|}{2\%}   & \multicolumn{1}{l|}{74\%}  & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{70\%}  & \multicolumn{1}{l|}{TLE}   & \multicolumn{1}{l|}{82\%}     & \multicolumn{1}{l|}{100\%} & 100\%                   \\ \hline
% click-tab-2-hard            & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{30\%}  & \multicolumn{1}{l|}{14\%}  & \multicolumn{1}{l|}{30\%}  & \multicolumn{1}{l|}{TLE}   & \multicolumn{1}{l|}{TLE}   & \multicolumn{1}{l|}{22\%}     & \multicolumn{1}{l|}{68\%}  & 0\%                     \\ \hline
% click-tab2-easy             & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{82\%}  & \multicolumn{1}{l|}{92\%}  & \multicolumn{1}{l|}{94\%}  & \multicolumn{1}{l|}{84\%}  & \multicolumn{1}{l|}{86\%}  & \multicolumn{1}{l|}{92\%}     & \multicolumn{1}{l|}{96\%}  & 95\%                    \\ \hline
% click-tab2-medium           & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{48\%}  & \multicolumn{1}{l|}{36\%}  & \multicolumn{1}{l|}{48\%}  & \multicolumn{1}{l|}{TLE}   & \multicolumn{1}{l|}{TLE}   & \multicolumn{1}{l|}{60\%}     & \multicolumn{1}{l|}{52\%}  & 28\%                    \\ \hline
% click-tab-2                 & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{14\%}  & \multicolumn{1}{l|}{4\%}   & \multicolumn{1}{l|}{28\%}  & \multicolumn{1}{l|}{TLE}   & \multicolumn{1}{l|}{TLE}   & \multicolumn{1}{l|}{44\%}     & \multicolumn{1}{l|}{78\%}  & 0\%                     \\ \hline
% click-tab                   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 99\%                    \\ \hline
% click-test-transfer         & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 100\%                   \\ \hline
% click-test-2                & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 100\%                   \\ \hline
% click-widget                & \multicolumn{1}{l|}{2\%}   & \multicolumn{1}{l|}{96\%}  & \multicolumn{1}{l|}{96\%}  & \multicolumn{1}{l|}{98\%}  & \multicolumn{1}{l|}{94\%}  & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{97\%}     & \multicolumn{1}{l|}{98\%}  & 96\%                    \\ \hline
% enter-date                  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 100\%                   \\ \hline
% enter-password              & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{96\%}  & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100.00\%} & \multicolumn{1}{l|}{100\%} & 100\%                   \\ \hline
% enter-text-dynamic          & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 98\%                    \\ \hline
% enter-text-2                & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{90\%}  & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{96\%}  & \multicolumn{1}{l|}{96\%}  & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 100\%                   \\ \hline
% enter-text                  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 100\%                   \\ \hline
% enter-time                  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{52\%}  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{98\%}  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{80\%}  & \multicolumn{1}{l|}{0\%}      & \multicolumn{1}{l|}{100\%} & 51\%                    \\ \hline
% focus-text-2                & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{78\%}  & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 100\%                   \\ \hline
% focus-text                  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{92\%}  & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 100\%                   \\ \hline
% guess-number                & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{32\%}  & \multicolumn{1}{l|}{8\%}   & \multicolumn{1}{l|}{14\%}  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{20\%}     & \multicolumn{1}{l|}{84\%}  & 14\%                    \\ \hline
% login-user                  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{96\%}  & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 100\%                   \\ \hline
% grid-coordinate             & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{86\%}  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{TLE}   & \multicolumn{1}{l|}{0\%}      & \multicolumn{1}{l|}{100\%} & 0\%                     \\ \hline
% simple-arithmetic           & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{90\%}  & \multicolumn{1}{l|}{97\%}  & \multicolumn{1}{l|}{90\%}  & \multicolumn{1}{l|}{90\%}  & \multicolumn{1}{l|}{100\%}    & \multicolumn{1}{l|}{100\%} & 99\%                    \\ \hline
% simple-algebra              & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{2\%}   & \multicolumn{1}{l|}{55\%}  & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{84\%}  & \multicolumn{1}{l|}{90\%}  & \multicolumn{1}{l|}{80\%}     & \multicolumn{1}{l|}{100\%} & 95\%                    \\ \hline
% navigate-tree               & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{32\%}  & \multicolumn{1}{l|}{51\%}  & \multicolumn{1}{l|}{94\%}  & \multicolumn{1}{l|}{60\%}  & \multicolumn{1}{l|}{74\%}  & \multicolumn{1}{l|}{70\%}     & \multicolumn{1}{l|}{92\%}  & 25\%                    \\ \hline
% search-engine               & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{6\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}      & \multicolumn{1}{l|}{20\%}  & 0\%                     \\ \hline
% find-word                   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{100\%} & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{44\%}  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{18\%}  & \multicolumn{1}{l|}{0\%}      & \multicolumn{1}{l|}{0\%}   & 0\%                     \\ \hline
% email-inbox-forward-nl-turk & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{85\%}  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{77\%}  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}      & \multicolumn{1}{l|}{92\%}  & 0\%                     \\ \hline
% email-inbox-forward-nl      & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{80\%}  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{97\%}  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}      & \multicolumn{1}{l|}{96\%}  & 0\%                     \\ \hline
% email-inbox-nl-turk         & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{11\%}  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{22\%}  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}      & \multicolumn{1}{l|}{18\%}  & 0\%                     \\ \hline
% email-inbox                 & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{20\%}  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{21\%}  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}      & \multicolumn{1}{l|}{21\%}  & 0\%                     \\ \hline
% email-inbox full example*   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{96\%}  & \multicolumn{1}{l|}{N/A}   & \multicolumn{1}{l|}{98\%}  & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{N/A}      & \multicolumn{1}{l|}{N/A}   & 0\%                     \\ \hline
% terminal                    & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}   & \multicolumn{1}{l|}{0\%}      & \multicolumn{1}{l|}{93\%}  & 0\%                     \\ \hline
%\end{tabular}}
%end{table}



\begin{lstlisting}[language=Python,basicstyle=\tiny, caption=function description, label={lst:fm},belowskip=-0.8 \baselineskip]
Function_Description = """
You should only use the functions provided herewith in the function description. 
Here is the list for the pre-defined functions [click_action1, enter_text_action, coord_click_action]

To use a function, please refer to the Name, Input, Output, Description of the functions, and usage examples below. Action functions should be called correctly in the solution. 

Function Name: click_action1
Input: tag or element, id or text, observation
Output: create_click_element_action
Description: useful when you want to click on an element in the web interface. This functions cannot be generalized on names. Normally first input is one of tag or element and second is test or id. The output is given as the action by calling click_action1 function or 'Cannot find in the DOM_element' if no such thing to be clicked on.
Example: Objects in Image: Button One;
         Task: Click button ONE;
         Solution: action = click_action1('button', 'ONE', observation)
                   observation, reward, terminated, truncated, info = env.step(action)

Function Name: enter_text_action
Input: input_text, observation
Output: create_type_action
Description: useful when you want to type the input_text into input text box or a similar object like input_number that can accept text given the observation of the task interface. Need to call click_action1 to click on it before calling this function. The output is given as the action by calling enter_text_action function.
Example: Objects in Image: input_text textbox; 
         Task: Type 'Hello' into textbox;
         Solution: ction = click_action1('input_text', 'textbox', observation)
                   observation, reward, terminated, truncated, info = env.step(action)
                   action = enter_text_action('Hello', observation)
                   observation, reward, terminated, truncated, info = env.step(action)
            
Name: scroll_action1
Description: needed when elements do not appear on initial screen. Always used with other actions
Example: Objects in Image: Button Apple 
         Task: scroll and click button Apple
         Solution: action = scroll_action1(text='Apple',observation)
                   observation, reward, terminated, truncated, info = env.step(action)
                   action = click_action1('button','Apple',observation)
                   observation, reward, terminated, truncated, info = env.step(action) 
"""
\end{lstlisting}




\subsection{Full API}
As described in the paper, we have defined a set of functions that allow our LLM to interact with the MiniWob++ environment. The functions reference the Selenium API. We use an additional function, called  also used a function called Furthermore, we have also developed a function that filters the DOM elements from the complete set. A summary of those APIs has been provided as a reference for their structure and functionality. In this section, we present a detailed implementation for each of those APIs listed below.

\begin{lstlisting}[language=Python,basicstyle=\tiny, caption=Full implementation of our API, label={lst:API},belowskip=-0.8 \baselineskip]
def getSummary(dom_elements):
    ''' 
    # get the filtered DOM elements from full DOM elements
    Input: DOM elements
    Output: Subset of DOM elements
    Example: # get the filtered DOM elements from the full one
             objects_in_the_image = getSummary(dom_elements)
    '''
    
def click_action1(tag_class_name,id_text_name,observation):
    '''
    # click on an specific element shown in the web interface
    Input: tag or element, id or text, observation
    Output: clicks on specific element in environment
    Example: # click on tab a
             action = click_action1('tab', 'a', observation)
             observation, reward, terminated, truncated, info = env.step(action)
    '''
    
def enter_text_action(input_text,observation):
    '''
    # enter text into a selected element shown in the web interface
    Input: text, observation
    Output: enters text in element in environment
    Example: # enter text 'neurips' into input_text textbox
             action = enter_text_action('neurips', observation)
             observation, reward, terminated, truncated, info = env.step(action)
    '''
    
def scroll_action1(text_to_scroll_to, observation):
    '''
    # scroll to the element that does not appear initially on web interface
    Input: text, observation
    Output: moves webpage such that certain text is visible
    Example: # scroll to button one
             action = scroll_action1(text='one',observation)
             observation, reward, terminated, truncated, info = env.step(action)
    '''
\end{lstlisting}
